Applications of the Octet Baryon Quark-Meson Coupling Model to Hybrid Stars

In this study we have investigated a particular state-of-the-art model which is currently used to refine our knowledge of the workings of the strong interaction and the way that it is manifested in both neutron stars and heavy nuclei, although we have placed emphasis on the former for reasons of personal interest. The main body of this work has surrounded an effective field theory known as Quantum Hadrodynamics (QHD) and its variations, as well as an extension to this known as the Quark-Meson Coupling (QMC) model, and variations thereof. We further extend these frameworks to include the possibility of a phase transition from hadronic matter to deconfined quark matter to produce hybrid stars, using various models. We have investigated these pre-existing models to deeply understand how they are justified, and given this information, we have expanded them to incorporate a modern understanding of how the strong interaction is manifest.

==> Chapter7_conclusions.tex <==
\chapter{Conclusions}\label{sec:conclusions}
%
%

